The Geometry of Numerical Reasoning: Language Models Compare Numeric Properties in Linear Subspaces

This paper investigates whether large language models (LLMs) utilize numerical attributes encoded in a low-dimensional subspace of the embedding space when answering questions involving numeric comparisons, e.g., Was Cristiano born before Messi? We first identified, using partial least squares regression, these subspaces, which effectively encode the numerical attributes associated with the entities in comparison prompts. Further, we demonstrate causality, by intervening in these subspaces to manipulate hidden states, thereby altering the LLM's comparison outcomes. Experiments conducted on three different LLMs showed that our results hold across different numerical attributes, indicating that LLMs utilize the linearly encoded information for numerical reasoning.

==> analysis.tex <==
\label{sec: error analysis}


\subsection{Observations from Experiment 1}
\textbf{Observation 1.} From Experiment~\ref{experiment1} we can find that the Mean absolute error is about $10$ years, meaning that the model prediction always falls in the same century as the true birth year. 



\textbf{Observation 2.} We can see also observe that the model failed to predict the negative birth year(i.e., BC) for instance the model almost correctly predicted the birth year of Moses but without the negative sign: \textit{When Was Moses Born? give the year of birthdirectly do not output any additional information.}, the model output: $1392$. The correct answer is $-1393$. One possible reason for this, is maybe because we are asking the model to output only the birth year, so maybe if we gave the model more freedom, it will output something like \textit{$1392$ BC}

\textbf{Observation 3.} One of the failures of the model, is in predicting the birth year of fictional characters if it is in the future. For instance the model predicted that the birth year of Nyota Uhura(character from Star Treck) is in $1946$, while the true birth year is in $2233$.

\textbf{Observation 4.} We are using birth dates extracted from Wikipedia, however other resources may have different birth years of the tested entities. We notice that the model struggle with this types of historical enitites. For instance when we ask the model about the birth year of \textit{Adriaen Hanneman}, the model outputs $1610$, this is different from the date in Wikipedia($1603$), but further investigation into other resources~\footnote{\url{https://www.nationalgalleries.org/art-and-artists/artists/adriaen-hanneman?__cf_chl_tk=l4fK5e6ACkBuZ1XAZ8KvrwUFQ8f21WPr7PQloQSYYrk-1719832388-0.0.1.1-3839}}
revel that its birth year maybe $1911$ which is closer to the model prediction.

\textbf{Observation 5.} Not correct dates in Wikipedia. In some instances the model outputs a correct date that are different than the ones in the test datsets. For instance, the dataset with have claim that \textit{Timothy Dalton} was born in $1944$ while this Wikipedia page~\footnote{\url{https://en.wikipedia.org/wiki/Timothy_Dalton}} and our model say it is $1946$



\subsection{Observations from Experiment 2}

\textbf{Observation 1}


